Metric Program Synthesis

We present a new domain-agnostic synthesis technique for generating programs from input-output examples. Our method, called metric program synthesis, relaxes the well-known observational equivalence idea (used widely in bottom-up enumerative synthesis) into a weaker notion of observational similarity, with the goal of reducing the search space that the synthesizer needs to explore. Our method clusters programs into equivalence classes based on a distance metric and constructs a version space that compactly represents "approximately correct" programs. Then, given a "close enough" program sampled from this version space, our approach uses a distance-guided repair algorithm to find a program that exactly matches the given input-output examples. We have implemented our proposed metric program synthesis technique in a tool called SyMetric and evaluate it in three different domains considered in prior work. Our evaluation shows that SyMetric outperforms other domain-agnostic synthesizers that use observational equivalence and that it achieves results competitive with domain-specific synthesizers that are either designed for or trained on those domains.

==> cad.tex <==
\section{Instantiating Metric Synthesis for Inverse CSG}

\subsection{Distance Function}

CAD programs have three kinds of intermediate value: scenes, integers, and floats. Scenes are Boolean matrices that represent a rasterization of the underlying shapes. Integers are passed as counts to the \texttt{Repeat} operator, and floats in $[0,1]$ are used to write coordinate vectors.

The Jaccard distance is used as the metric for scenes. The constant function returning $\infty$ is used as the metric for integer and float values. This means that only scenes can be grouped together.

\todo{
	\begin{itemize}
		\item We use a different metric for deciding similarity between scenes that takes the target into account
		\item Need to explain why this is an improvement over the jaccard distance (with benchmarks?) and definitely a diagram
		\item Use the castle diagram
	\end{itemize}
}

\subsection{Constant tuning}

The performance of the algorithm is improved if a hill-climbing algorithm is used to tune the coordinates in the CAD program as a final step. Tabu search is the specific algorithm used. The neighbors of a program are that program with one of its floating point constants incremented or decremented (the floating point constants in the DSL are quantized, so this is a well-defined operation). This local search increases the probability that the program found will be exactly correct rather than close to correct.

\todo{
	The local search is a key part of the algorithm and we need to figure out how to describe it in a way that isn't specific to the CAD DSL. It should be related to the ways in which the DSL is continuous.
}

\subsection{Symmetry Breaking}

Although the existence of symmetric programs does not make the generation of the XFTA more expensive, it does make searching the resulting graph more difficult because it increases the number of paths that reach each state.

To address this issue, we define a \emph{canonical form} for CAD programs and modify the evaluation function to return $\bot$ for non-canonical programs. Furthermore, programs which evaluate to $\bot$ are not included in the XFTA.\@

\input{fig_canon}

The canonical form does not admit empty primitive shapes or primitive shapes that overlap the edge of the canvas. \texttt{Repeat} operators must move the shape and perform more than one repetition. The arguments to commutative operators like union must be in some order (any ordering will do).

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig_bottom_up.tex <==
\begin{figure}
	\begin{align*}
		P_0  & = \{ op() ~|~ op \in ops \}                                                               \\
		P_i' & = \{ op(p, q) ~|~ p, q \in P_{i - 1} \} \cup P_{i - 1}                                    \\
		P_i  & \subseteq P_i' \land (\forall p \in P_i.\ p \in P_i' \lor \exists q \in P_i.\ p \equiv q)
	\end{align*}\label{fig:bottom-up}
	\caption{Sketch of the bottom-up enumeration with equivalence reduction algorithm.}
\end{figure}


==> fig_canon.tex <==
% \begin{noindent}
\begin{algorithm}[!t]
  \begin{align*}
    \textsc{WF}(\texttt{Circle}(x, y, r))
    & = r > 0 \land 0 \leq x - r \land x + r < x_{max} \land 0 \leq y - r \land y + r < y_{max} \\
    \textsc{WF}(\texttt{Rect}(x_{1}, y_{1}, x_{2}, y_{2}))  & = x < x' \land y < y' \\
    \textsc{WF}(e - e') & = \textsc{WF}(e \cup e') = \textsc{WF}(e) \land \textsc{WF}(e') \\
    \textsc{WF}(\texttt{Repeat}(e, v, c)) & = \|v\| > 0 \land c > 1 \land \textsc{WF}(e)
  \end{align*}
  \caption{Algorithm for checking that a CSG program is well-formed.}\label{fig:well-formed}
\end{algorithm}
% \end{noindent}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig_generated.tex <==
\begin{figure}
	\includegraphics[width=0.8\textwidth]{generated.pdf}
\end{figure}


==> fig_main_table.tex <==
\begin{table}
	\input{main_table}
	\caption{Comparison of \name against existing synthesis algorithms. Each benchmark can either succeed or fail due to timeout, memory exhaustion, or in the case of \textsc{FTA-Syngar} (NR) because the benchmark is unsatisfiable without the \texttt{Repeat} operator. Runtimes are given in seconds, and are only shown for the benchmarks that succeeded. All benchmarks are run with a 1 hour timeout and 4GB of memory.}\label{tbl:eval}
\end{table}


==> problem.tex <==
\section{Problem Statement}

We frame the inverse CSG problem as instance of example-based program synthesis. The input to the synthesizer is a bitmap image and the output is a program in the target CAD domain-specific language.  In the remainder of this section, we present the DSL for this domain and formalize the synthesis problem. 




\subsection{Domain-Specific Language for Inverse CSG}

\input{fig_grammar}

\Cref{fig:syntax} shows the syntax of the domain-specific language in which we synthesize programs. This DSL includes two primitive shapes, namely circles and rectangles. Circles are represented by a center coordinate and a radius. Rectangles are axis-aligned and are represented by the coordinates of the lower left and upper right corners. These primitive shapes can be combined using union, difference, and repeat operators. In particular, 
  $\texttt{Repeat}(E, x, y, c)$ takes a scene $E$, a translation vector $v = (x, y)$, and a count $c$, and  it produces the union of $E$ repeated $c$ times, translated by $v$. For example, we have: $$\texttt{Repeat}(\texttt{Circle}(v, r), v', 2) = \texttt{Circle}(v, r) \cup \texttt{Circle}(v + v', r)$$
  \texttt{Repeat} allows programs with repeating patterns to be expressed compactly, which also makes these programs easier to synthesize.

%Coordinate values are quantized to the range [0, 16), and repetition counts are limited to the range [2, 5).

%\subsection{Semantics}

\Cref{fig:semantics} presents the semantics of our  CAD DSL using an {\sc Eval} procedure, which takes as input a program and produces a bitmap image. Specifically, we represent a bitmap image as a mapping from each pixel $(u, v)$ to a boolean indicating whether that pixel is filled or not, or equivalently as the set of all pixels that evaluate to true.   Given a program $P$ in our DSL, we use the notation $\eval{P}$ to denote the bitmap image produced by $P$.

% evaluate to predicates of the form $\mathbb{R}^2 -> \mathbb{B}$. A CAD program will return true for points that are contained in the output shape, and return false for points that are outside the shape. However, we consider a CAD program $P$ to be correct for some input bitmap $B$ if $\forall 0 \leq x, y < 16.\ B[x, y] = P(x, y)$.

\input{fig_semantics}

\subsection{Synthesis Problem}

 Given a bitmap image $B$, represented as a mapping from pixels $(x, y)$ to  booleans, inverse CSG is the problem of synthesizing a program $P$ such that the following condition holds:
\[
\forall x, y \in \emph{Domain}(B). \ B(x, y) = \eval{P} (x, y)
\]

Viewed in this light, note that inverse CSG is exactly a programming-by-example (PBE) problem: We can think of the bitmap image as a set of I/O examples where each input example is a pixel $(x, y)$ and the output example is a boolean. Then, the inverse CSG problem aims to synthesize a program $P$ in our DSL that is consistent with all of these examples. However, a key difference from standard PBE is that the number of examples we need to deal with is quite large: for instance, in our evaluation, we use $32 \times 32$ bitmap images, so the number of I/O examples is 1024. 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> regex_construct_times.tex <==

\begin{tabular}{lrrrrrr}
\toprule
Benchmark & \multicolumn{2}{c}{Expansion} & \multicolumn{2}{c}{Clustering} & \multicolumn{2}{c}{Ranking} \\
& Median & Max & Median & Max & Median & Max \\
\midrule

All & 0.3 & 280.6 & 0.0 & 4.3 & 0.0 & 0.7 \\
\bottomrule
\end{tabular}


==> regex_method_times.tex <==

\begin{tabular}{lrrrrrr}
\toprule
Benchmark & \multicolumn{2}{c}{\textsc{ConstructXFTA}} & \multicolumn{2}{c}{\textsc{Extract}} & \multicolumn{2}{c}{\textsc{Repair}} \\
& Median & Max & Median & Max & Median & Max \\
\midrule

All & 0.7 & 281.9 & 0.0 & 18.8 & 0.0 & 195.1 \\
\bottomrule
\end{tabular}


==> towers_construct_times.tex <==

\begin{tabular}{lrrrrrr}
\toprule
Benchmark & \multicolumn{2}{c}{Expansion} & \multicolumn{2}{c}{Clustering} & \multicolumn{2}{c}{Ranking} \\
& Median & Max & Median & Max & Median & Max \\
\midrule

All & 4.8 & 139.6 & 0.4 & 10.3 & 0.0 & 0.0 \\
\bottomrule
\end{tabular}


==> towers_distance.tex <==
\section{Tower Building Distance in Detail}

We are particularly interested in how programs behave when they are placed inside a loop, so we gather the states by iterating the program. We define an approximate evaluation function $\textsc{Eval}_k$ that computes $k$ iterations of a program $P$ on the initial state $s_0:$ \[\textsc{Eval}_k(P) = \{\textsc{Eval}(P_1; \dots; P_i, s_0) ~|~ 1 \leq i \leq k\}.\]

To compute the distance between two tower programs $P$ and $P'$, we approximate them using $\textsc{Eval}_k$ yielding $q = \textsc{Eval}_k(P)$ and $q' = \textsc{Eval}_k(P')$. The distance between $P$ and $P'$ is then the average distance between the states in $q$ and $q'$. This distance is defined as: $\delta_T(q, q') = (\sum_i^k \delta_S(q_i, q'_i))/k.$ 

As discussed in~\Cref{sec:tower-dist}, the purpose of the distance $\delta_T$ is to determine whether two programs are similar enough that they should be treated as equivalent during the search. The distance from a program $P$ to the goal is a measure of the \emph{usefulness} of $P$, either as a solution or as a subprogram in some eventual solution. Therefore, we treat the distance between a program and the goal slightly differently than we treat the distance between programs. 

First, we want to determine if $P$ is a useful subprogram. We often want to build multiple towers side-by-side, which means that the individual towers are likely to be useful subprograms. We incorporate this idea into our distance measure by dividing the goal into its component towers. We perform this division by taking a series of vertical slices of the goal. For each $0 \leq i \leq x_{max},$ we define two slices consisting of the blocks with an x-position less than and greater than $i$. A slice at $i$ is valid only if there are no horizontal blocks that overlap $i$. For a goal $G$, we let $\vec{G}$ be the slices. Note that the original goal is in $\vec{G}$.

Now we can define the distance between a program $P$ and the goal $G$. The distance between $P$ and $\vec{G}$ is \[\delta_G(\vec{G}, q) = \min_{g \in \vec{G}, s\in q} \delta_S(g, s) + |G - g|,\] which gives the minimum distance between $q$ and one of the vertical slices, with a penalty $|G - g|$ for the blocks that are not in the slice. Finally, we let $p_r > 1$ in $\delta_G$, which reflects the fact that blocks that are present in $q$ but not in $G$ should be penalized more than blocks that are missing in $q$.


==> towers_method_times.tex <==

\begin{tabular}{lrrrrrr}
	\toprule
	Benchmark & \multicolumn{2}{c}{\textsc{ConstructXFTA}} & \multicolumn{2}{c}{\textsc{Extract}} & \multicolumn{2}{c}{\textsc{Repair}}                      \\
	          & Median                                     & Max                                  & Median                              & Max & Median & Max \\
	\midrule

	All       & 9.1                                        & 171.8                                & 0.0                                 & 0.0 & 0.0    & 0.0 \\
	\bottomrule
\end{tabular}

